On the Feasibility of Exploiting Traffic Collision Avoidance System Vulnerabilities

Traffic Collision Avoidance Systems (TCAS) are safety-critical systems required on most commercial aircrafts in service today. However, TCAS was not designed to account for malicious actors. While in the past it may have been infeasible for an attacker to craft radio signals to mimic TCAS signals, attackers today have access to open-source digital signal processing software, like GNU Radio, and inexpensive software defined radios (SDR) that enable the transmission of spurious TCAS messages. In this paper, methods, both qualitative and quantitative, for analyzing TCAS from an adversarial perspective are presented. To demonstrate the feasibility of inducing near mid-air collisions between current day TCAS-equipped aircraft, an experimental Phantom Aircraft generator is developed using GNU Radio and an SDR against a realistic threat model.

==> Notes/Berkay-notes.tex <==

Basavesh Thoughts: I kind of read the whole thesis skimming few parts related to protocol and some block diagrams. As we previously discussed, it explains how we can induce 2 aircrafts (X & Y) to collide each other by jamming the (Y) first and then Spoofing messages such that there is a Ghost/Phantom/Spoofed aircraft is approaching X and advocates X to go through the Y path and cause a collision using Software Defined Radio Technology.

==> backup/Implementation/impl.tex <==
\section{Attack Implementation}
\label{sec:attack-implementation}
We demonstrate the developed attack  platform that uses GNU Radio as the foundation of its architecture.  We present the block diagrams of the platform and the methods for simulation. Lastly, an outline of the hardware used for this platform is presented.



\subsection{Phantom Aircraft Generator}
We demonstrate a proof-of-concept that a GNU Radio application can bait a TCAS into surveying the phantom aircraft platform. Our goal is to have a pair of zero-speed aircraft track each other. This is sufficient for the proof-of-concept because the core functionality of an attacker and a normal aircraft are identical. We refer this design to a phantom aircraft generator.

\begin{figure}[t!]
    \centering
    \includegraphics[width=8cm, keepaspectratio]{block_overview.jpg}
    \caption{Overview block diagram of the phantom aircraft generator.}
    \label{fig:blockDiagramOverview}
\end{figure}

We design the system as modular as possible within the GNU Radio ecosystem and build upon other Open-Source GNU Radio modules. The Python(2.7.12) module Out-of-Tree (OOT) created for the paper is called \textit{gr-modes}. It contains custom aircraft application code and modules that are designed to aid in message transformations. The reception and demodulation of DF packets is handled by \textit{gr-adsb} (ADS-B OOT for GNU Radio)~\cite{misc:gh_adsb}. The total OOT dependencies for gr-modes are: (1) \texttt{gr-adsb}: demodulation and decoding of ADS-B messages~\cite{misc:gh_adsb}, (2) \texttt{gr-burst}: blocks for building PSK modems \cite{misc:gh_burst}, (3) \texttt{gr-eventstream} \cite{misc:gh_eventstream}, (4) \texttt{gr-mapper} \cite{misc:gh_mapper}, and (5) \texttt{gr-pyqt} \cite{misc:gh_pyqt}

Universal Software Radio Peripheral (USRP) hardware requires significant processing power in general, especially at high sample rates.  The PC for the attack uses an Intel Core i7-6800K; it has six cores at a 3.4 GHz clock rate.  Combined with 16 GB of RAM, this PC provides adequate flexibility in processing two USRPs simultaneously. Two USRPs act like a pair of communicating TCAS.  An Ettus Research B210 is the transmitting USRP, and an Ettus Research N210 is the receiving USRP~\cite{manual:b210, manual:n210}.  Both USRPs have programmable FPGAs which enables better performance if software alone is insufficient for some function.  The N210 only has a single pair of SMA-bulkheads which must be accounted for in a full test of TCAS; this can be solved by either introducing power combiners or by switching SDR platform (e.g. using an identical B210). The two USRPs communicate over SMA cables through a variable attenuator.  The attenuator prevents the receiver's analog to digital converter (ADC) from being saturated.  The N210 communicates with the PC over 10 Gbps Ethernet, and the B210 communicates over a USB 3.0 port.

\subsection{Phantom Aircraft Attack Details}
We present the architecture of phantom aircraft generator software system, the sub-routines of each high-level block, and the interfaces between each function. 

Our system uses a mixture of  asynchronous and streamed data. We require four RF interfaces: a TX and RX interface for both interrogations and replies.  The interfaces do not use the normal frequencies bands of TCAS~\cite{manual:annex10_vol4, manual:acas_manual, manual:intro_tcas_ii}.  Instead, a nearby carrier frequency in the industrial, scientific, and medical (ISM) band is chosen to open the opportunity for wireless testing~\cite{manual:ism_bands}.  Each RX interface has its own set of blocks that have the task of converting raw samples into packets the \texttt{Core Logic} can understand; each TX interface performs the conversion in the opposite direction.  The range estimation occurs from the RTT of the interrogation-reply cycle. For estimation of RTT, the UF TX blocks feedback a timestamp to the \texttt{Core Logic}. The elapsed time is calculated from a timestamp delivered by the DF RX blocks upon receipt.  The overview supports a jamming interface from the \texttt{core logic}. The core logic would \texttt{enable} or \texttt{disable} the jam for an arbitrary amount of samples. The jamming signal generator handles the generation of a random samples independent of the \texttt{core logic}. 

All communication interfaces support unpacked bytes.  For the purpose of this design, this means that an 8 bit sample can only hold the value of a binary one or binary zero. While inefficient in its memory usage, this design choice does make the design of other components--especially \texttt{lambda function} blocks~\cite{manual:lambda_functions}--much simpler. Conversion of data from the \texttt{Core Logic} to samples interface also handles the packing of message data into a complete Mode S message. A \texttt{lambda function} block from \texttt{gr-pyqt} and a \texttt{prepend preamble} block from \texttt{gr-burst} are convenient for packing the data into a Mode S reply~\cite{misc:gh_pyqt, misc:gh_burst}.  

The data that enters the DF TX interface from the \texttt{Core Logic} is 56 or 112 samples of bytes in length (although this interface is designed to be independent of payload size). To convert this message into a Mode S reply, the following procedure is performed: (a) Pulse Position Modulation (PPM) is performed on each sample~\cite{art:ppm}, (b) the Mode S reply preamble (a constant 16 sample vector with 1 sample per symbol assumed) is attached to the beginning of the packet, and (c) the packet is interpolated to the application's base sample rate. Then, the packet must be converted to a \textit{stream} of complex samples because GNU Radio only supports transmitting data over USRP that is in 32 bit complex stream format. Once the payload is packed into a complete Mode S reply, \texttt{gr-eventstream} is used to insert the data from an \textit{asynchronous} packet into the sample stream, and conversion to a 32 bit complex type is performed with conversion blocks.

The receiver interface for DF messages is made from \texttt{gr-adsb} blocks, which expect squared magnitude 32 bit float samples~\cite{misc:gh_adsb}. The \texttt{ADS-B Framer} is slightly modified such that the \texttt{ADS-B Framer} block creates a timestamp that propagates to the \texttt{Core Logic} when a preamble is detected.  The \texttt{ADS-B Framer} block correlates the input with the expected preamble and creates a \texttt{tag} object on the first sample of the preamble when a match is detected.  This \texttt{tag} serves as the synchronization point which the \texttt{ADS-B Demodulator} can use for PPM demodulation.  The decoder in the \texttt{gr-adsb} OOT module is bypassed entirely, and the asynchronous output is sent directly to the \texttt{Core Logic} for custom decoding routines. We mimic the design of the reply transmission interface such that the interface remains independent of actual message data. However, some adjustments have to be made to support the different pulse sequence and modulation scheme of Mode S interrogations. Namely, Mode S interrogations have slightly more padding than replies. There is a two sample pad of zeros (assuming 1 sample per symbol) appended to the end of the message payload, and a seven sample preamble is attached to the message.  The preamble is structured such that one phase shift occurs at the exact point labeled ``Sync. Phase Reversal"~\cite{manual:annex10_vol4} after the preamble is put through Differential Binary Phase Shift Keyed (DBPSK) modulation.

Separate from the preamble that contains the ``Sync. Phase Reversal", another preamble is attached to the output of the DBPSK modulator.  This second preamble suppresses Modes A and C transponders from processing the interrogation.  The interval between the first and second pulse dictates how Modes A and C transponders reply (if at all) to an interrogation~\cite{manual:annex10_vol4}.  After the last preamble is inserted, the payload is finally transmitted and converted to a data stream format that the USRP expects. We note that the ``Side Lobe Suppression (SLS) control transmission`` is omitted in interrogations for simplification.  The purpose of this transmission is to prevent aircraft to the side or behind the aircraft from responding in special circumstances.  The SLS control is transmitted on a separate antenna and is designed to hide the ``Sync. Phase Reversal" of an interrogation, which prevents a Mode S transponder from synchronizing its incoming waveform~\cite{manual:annex10_vol4}.

The receiving interface for Interrogation Framer block performs correlation of the preamble and creates a \texttt{tag} on the first sample of the preamble. Using the aforementioned \texttt{tag} as a synchronization point, the \texttt{Tag Consumer} block then creates a ``slice" of samples.  The slice starts from the first sample of the DBPSK samples and ends 120 samples later (i.e. length of the preamble + 112 symbols assumed).  This slice is packaged into a format acceptable for asynchronous message passing, and then, demodulation is performed asynchronously.  Although a 112 symbol payload is assumed, the extraneous information packaged when a short message was actually received is tolerable because the core knows the true message size based on the fixed 5 symbol header.

 The receiving interfaces of the \texttt{Core Logic} convert interrogation and reply samples into a format the state machine logic can understand.   The conversion process is based off the routines of the \texttt{ADS-B Decoder} of the \texttt{gr-adsb} package.  Because of its fixed length, The header is decoded first to provide information about verifying the checksum in the final 24 bits of the payload. If the parity check passes, then the vector of samples is converted into a \texttt{downlink object} or \texttt{uplink object} depending on which interface is used. The \texttt{downlink} and \texttt{uplink} objects are provided by a Python module written for supporting the \texttt{Core Logic} functions.  The module provides classes for each message type as well as useful helping functions.  
 
The \texttt{state machine} blocks can be ``swapped" out to change the behavior of a phantom aircraft.  For this proof-of-concept, a simplified state-machine operation is used in this design. This aircraft simply detect nearby DF 11 messages and begin surveillance of the aircraft that transmitted the message. The classes for \texttt{downlink} and \texttt{uplink} objects automatically perform the construction of the vector and the parity check.  The only requirement of the user is to call the automatic conversion function, and then, they place the result of that routine into the output message queue.

\section{Evaluation}
\begin{comment}
I will delete this later.
\berkay{Can we improve this section little bit? It seems the results and explanations are very sparse. Can we use any content from thesis?}
\bash{I will look into Evaluation now, I was reading the whole part till now. I think the above part is logical and makes sense.} 
\berkay{Thanks. I will notify Virginia Tech folks around 2:30pm today. }
\bash{Sure.}
\end{comment}

We verify our attack detailed in Section~\ref{sec:attack-implementation}. If our design works as expected, then the generation of phantom aircraft is sufficiently verified. While the direct testing approach would be to generate aircraft on a real TCAS, real TCAS hardware is not trivial to acquire and setup.  Therefore, verification is completed when two simplified aircraft cores can track each other at zero speed through the medium of Mode S messages. We performed a series of unit tests and integration tests through GNU Radio to verify the adversarial tasks. We unit-tested all custom attack functionalities through GNU Radio's \texttt{gr\_unittest} framework before integration within GRC~\cite{manual:gr_manual}. For each point of verification below, we executed the flowgraph for 10 minutes with a fixed surveillance period of one second such that approximately 600 rounds of interrogations and replies occur for each item. We have verified the following:

\begin{enumerate}
    \item Arbitrary Mode S reply messages can be crafted to fool the \texttt{gr-adsb} receiver without USRP hardware in-the-loop~\cite{misc:gh_adsb}).
    
    \item The \texttt{gr-adsb} receiver's performance can be characterized via a packet-loss calculation with USRP hardware in-the-loop.
    
    \item Arbitrary Mode S interrogation messages can be crafted to fool a custom Mode S interrogation receiver without USRP hardware in-the-loop. 
    
    \item All four message modulators and demodulators can deliver payloads to the \texttt{core logic}. The core logic performance is indicative of the state machine functionality.  No USRP hardware is used in-the-loop.
\end{enumerate}


\begin{comment}
\begin{figure}[t!]
    \centering
    \includegraphics[width=8cm]{Images/verify_df_txrx_hw_bar.png}
    \caption{Graph of percent packet loss versus TX gain.}
    \label{fig:verify_df_txrx_hw_bar}
\end{figure}
\end{comment}


\begin{figure}[t!]
    \centering
    \includegraphics[width=8cm]{Images/verify_df_txrx_nohw_gui.jpg}
    \caption{Real-time graph showing the DF 17 message received and decoded.}
    \label{fig:verify_df_txrx_nohw_gui}
\end{figure}

\para{Mode S Reply}
We first verified that we correctly modulated, demodulated, and decoded a crafted payload message as shown in Figure~\ref{fig:verify_df_txrx_nohw_gui}. The message is also converted from asynchronous data into streamed data and back again such that synchronization is also tested. 
Second, we did performance evaluation of our software's susceptibility to packet loss. Six different 10-minute test runs are performed. For each test, the TX gain is noted. Then the amount of messages sent and received are counted. If a received message does not pass CRC check, we count it as a dropped packet. We found that even the best performing case still has a packet-loss factor nearly 60\%. While this is a significant problem for hardware testing, our main focus is its emulation of TCAS functionality. Therefore, the remainder of the tests ignore the use of USRP hardware. %From \ref{fig:verify_df_txrx_hw_bar},

\begin{figure}[t!]
    \centering
    \includegraphics[width=8cm]{Images/verify_uf_txrx_nohw_gui.jpg}
    \caption{Three real-time plots of the interrogation interface test.  The top plot shows the asynchronous TX bit stream, the middle plot shows the asynchronous RX bit stream, and the lower plot shows the real-time plot of the \texttt{framer} marking the start of the message.}
    \label{fig:verify_uf_txrx_nohw_gui}
\end{figure}

\para{Mode S interrogation} We verified that an arbitrary payload of 112 bits is modulated and demodulated to conform an expected Mode S interrogation. The message is converted from asynchronous data into streamed data and back again through a simulated Additive White Gaussian Noise (AWGN) channel as shown in Figure~\ref{fig:verify_uf_txrx_nohw_gui}. 


\para{Core Logic} We verified that the core logic demonstrates required states in software-only environment, which is sufficient for proving the base-level functionality of this phantom aircraft generator. We note that altitude information is as expected. However, the computational overhead is too large and imprecise for range estimation as shown in Figure~\ref{fig:verify_core_nohw_console}. Therefore, further investigation into improving the RTT estimation is required.
%what is this?

\begin{comment}
Discussion: (taken from thesis)
"The fourth and final test is shown in Section 7.2.4. However, the results of that verification
remain inconclusive because of the imprecise estimation of RTT. During the design of the
range estimator, it was assumed that the software could be sufficiently precise enough to
make accurate RTT estimations; this assumption is shown to be untrue, however. The
software cannot precisely estimate RTT in its current state, and other analytical approaches
have shown this approach to be problematic [66]."
\end{comment}

\section{Discussion}
The implementation of a non-malicious phantom aircraft generator is not fully realized yet. There is an opportunity to implement a more sophisticated spoofer with more significant real-time constraints by developing modules that more closely follow the GNU Radio idiosyncrasies, removing expensive message interfacing from the architecture, and possibly implementing a high-accuracy time-stamping in the SDR's FPGA. However, in the software’s current state, other more straightforward attacks are realizable because they do no rely on the attacker’s ability to create an accurate range estimate like the DoS attacks. Nevertheless, a sophisticated attack like the malicious Phantom Aircraft requires additional work to realize on an SDR.

TCAS is not found to be a secure system.  The difficulties had in attacking TCAS can be attributed to its nature as a highly complex system that is difficult to learn about--a phenomenon colloquially known as ``security through obscurity"~\cite{misc:obscurity}. However, obscure systems only have time as its defense; those with the time and resources to attack a complicated system will make it work eventually. Therefore, it is imperative that those who can defend these systems to use this time to their own advantage. 

As future work, it is also essential to develop a platform in which implementations can be tested on real TCAS hardware.  TCAS cannot operate independently from its inputs; it has subroutines which disable the TCAS if inputs are failing or nonexistent~\cite{manual:annex10_vol4, manual:acas_manual, manual:intro_tcas_ii}.  Therefore, designing a test bench in which TCAS can operate on real or simulated inputs would be invaluable to security work about it.

\begin{figure}[t!]
    \centering
    \includegraphics[width=8cm]{Images/verify_core_nohw_console.jpg}
    \caption{Imprecise RTT measurements from the design under test}   
    \label{fig:verify_core_nohw_console}
\end{figure}

==> backup/notes.tex <==
\begin{comment}
\begin{figure}[t!]
    \centering
    \includegraphics[width=8cm, keepaspectratio]{atktree_unres.jpg}
    \caption{A simplified version of the branch on \textbf{unresolved} NMAC in the TCAS attack tree.}
    \label{fig:atktree_unres}
\end{figure}

\para{Unresolved NMAC Attacks}
An unresolved attack attempts to increase the probability that two aircraft on a collision path do not maneuver in time to avoid NMAC. To fit the scope of this work, the simplified attack tree diagrams emphasize communications attacks. Figure~\ref{fig:atktree_unres} shows a section of the unresolved NMAC component.  In general, attacks that leave an NMAC unresolved are idealized to interfere with the TCAS communications in some way.  Specifically, attacks should focus on denying the 1090 MHz frequency band because reply messages on the 1090 MHz channel are necessary for maintaining a track against an intruder.  While jamming of the 1090 MHz channel is a simple example of a DoS attack that achieves the goal, arbitrary jamming attacks are not a noteworthy threat against TCAS because they are easily detected or thwarted \cite{art:jamming}. Instead, there are more effective approaches to garbling the 1090 MHz channel.  These types of attacks are classified under the Reply Channel Flood category of attacks in Figure \ref{fig:atktree_unres}.  Two examples of a reply channel flood are:
\begin{itemize}
    \item \textbf{All-Call Flood}:  The attacker abuses a special Mode S interrogation - the All-Call interrogation\cite{manual:annex10_vol4} - on the 1030 MHz channel to force all Mode S transponders that receive it to reply with its ICAO address.  This attack is more effective in higher traffic densities.
    \item \textbf{Squitter Flood}:  The attacker can pose as an aircraft by transmitting various All-Call reply messages on the 1090 MHz channel.  This attack takes advantage of the fact that TCAS passively monitors for nearby All-Call replies to reduce congestion of the 1030 MHz channel.  The attacker can utilize any address in the size $2^{24}$ ICAO address space to force nearby TCAS into continuously repeating the acquisition phase of intruder tracking without repeating false addresses~\cite{manual:acas_manual, manual:annex10_vol4}.
\end{itemize}

The main drawback to unresolved NMAC attacks is the reliance on an existing NMAC scenario. Flight data indicates that a plane would experience an NMAC approximately once every 100,000 flight hours on average~\cite{tech:minimum_tcas_ii_fta}.  From an adversarial perspective, it would be best if the adversary could cause NMACs arbitrarily.  A more powerful attack grants the full control of inducing NMAC at the attacker's will.

\end{comment}

==> backup/tcas_security.tex <==

\begin{comment}

\section{TCAS Security}
\subsection{TCAS FTA analysis}
TCAS runs safety-critical aeronautical software, is also required to demonstrate robustness to failure through compliance with the MOPS DO-178B~\cite{}. MITRE Corporation effort resulted a System Safety Study of Minimum TCAS II report to prove its impact on aeronautical safety~\cite{tech:minimum_tcas_ii_fta}. The TCAS safety study places emphasis on the limitations and failures of TCAS. In particular, the study explores how transponder equipage, altimetry errors, and sudden maneuvers affect the performance of TCAS. Then, the study addresses the failure mechanisms of surveillance, bit errors, avionics failures, etc. Finally, different scenarios involving pilot errors are also taken into account.

The study defines its undesired (or top) event as the result of faults which could cause two planes to result in a Near Mid-air Collision (NMAC). NMAC is defined as a scenario where two aircraft have a vertical separation of 100 ft or less and a horizontal separation of 500 ft or less. The study defines a term called risk ratio: a factor that describes the risk of encountering NMAC when equipped with a TCAS relative to the risk of encountering NMAC without a TCAS. In other words, a risk ratio of 1 would mean that the probability of experiencing NMAC is unchanged with the equipage of TCAS, a risk ratio less than 1 would mean the aircraft is more safe with TCAS equipped, and a risk ratio greater than 1 would indicate the aircraft is less safe with TCAS equipped.

%\subsubsection{Probability of encountering an NMAC}
To quantify a risk ratio of relative probability of NMAC, an estimate of the absolute probability of encountering an NMAC is required. Using flight data as well as incident reports from the FAA, some of the key discoveries of TCAS are:
\begin{itemize}
    \item 70\% of NMAC incidents occurred in bright daylight conditions. The study assumes visual acquisition is impossible for all other conditions.
    \item 16\% of NMAC incidents happened in Instrument Meteorological Conditions (IMC) [citations].
    \item The distribution of relative altitude amongst all CPA encounters is approximately uniform.
    \item The absolute probability of encountering an NMAC is estimated as 1 NMAC per 100,000 flight hours.
\end{itemize}

Some of the report findings would be unrealistic to model today. For example, the safety study found that of all NMAC encounters, 61\% of encounters involved aircraft with altitude reporting transponders. However, it can be speculated that the number of incidents involving altitude-reporting transponders would be closer to the total number of transponders in service: 92\%. 

\input{tables/fta_basic_original.tex}

\input{tables/fta_human_vars.tex}

%TCAS is dependent on a well-trained pilot properly maneuvering on TCAS instructions. Therefore, it is worthwhile to also associate plausible mistakes the pilot may make with the FTA, thereby converting the original FTA into a fuzzy-logic FTA [citation]. Table [ref] summarizes five human failures that can arise from visual, RA, and TA information [citation].



%\para{NMAC failure categories}
After exploring the TCAS environment, an FTA can relate the probability NMAC to relevant TCAS failures. NMAC failures are qualitatively categorized into two mutually-exclusive failure modes. These modes are defined as:
\begin{itemize}
    \item \textbf{Unresolved NMAC}: Two planes are already on a collision course, and the pilots fail to maneuver the planes in a way that avoids NMAC.
    \item \textbf{Induced NMAC}: Two planes that were not previously on course towards NMAC are maneuvered into a NMAC.
\end{itemize}


The study further explores the limitations and failure mechanisms of TCAS. Table \ref{tab:fta_basic_original} describes these basic probabilities and attaches an identifier to each condition.  Some of these basic probabilities could be modified when considering the adversary.  For example, if an attacker could force TCAS into releasing an RA without any visible aircraft nearby, events \texttt{n} and \texttt{o} would become 1 since there is no aircraft for a pilot to visually acquire. Another important failure component is the pilot.  TCAS is dependent on a well-trained pilot properly maneuvering on TCAS instructions.  Therefore, it is worthwhile to also associate plausible mistakes the pilot may make with the FTA, thereby converting the original FTA into a fuzzy-logic FTA \cite{art:fuzzy_fta}. Table \ref{tab:fta_human_vars} summarizes five human failures that can arise from visual, RA, and TA information \cite{tech:minimum_tcas_ii_fta}. 

With basic events and human failures defined, a formulation for the top event is possible.  However, the full fault tree shown in \cite{tech:minimum_tcas_ii_fta} is very complicated, and certain sub-branches can be simplified if some nominal operating conditions are assumed.  After the formulation is made, the assumptions made in the nominal conditions can be adjusted in a sensitivity analysis. These nominal operating conditions are: (a) Pilots will always avoid planes they can see, (b) If there is no opportunity to visually acquire the threat, the pilot will follow the RA, (c) Visual acquisition is only possible in bright daylight, (d) The intruder is not TCAS-equipped, and (e) Bad maneuvers are not made by the TCAS pilot.

%The component of particular interest is the induced component of NMAC because the induced component is antithetical to the design goals of TCAS. As an adversary, demonstrating control over the induced NMAC component would imply that an attacker could arbitrarily redirect two nearby planes into each other.

\para{Unresolved Component} The unresolved component of all NMACs is comprised of nine failure modes. Each of these components are summed as the total unresolved component. Some events have human factors associated with their probabilities. Each human factor is represented as a variable, where the variable corresponds to the labels outlined in Table~\ref{tab:fta_human_vars}. The failure rate for the unresolved component is defined as:
\scalebox{0.86}{$P_u = 0.413 + 0.259( \mathit{VNA} + \mathit{TNA} ) + 0.327 ( \mathit{RNF} ) + 0.0008 (\mathit{VMIR} ) $}

\para{Induced Component.} The induced component is only comprised of five failure modes. Their sum results in the total probability of the induced component. Some events that make up the induced component are also dependent on human failures. 
The failure rate for the induced component is defined as: \scalebox{0.99}{ $ P_i = 0.11 + 0.014 (\mathit{VMIR}) + 0.59 (\mathit{TI})$}

\para{Top Event.} The top event is simply the sum of the two major components because the induced component
is mutually exclusive from the unresolved component. This top event probability,  $P = P_u + P_i$, is therefore fully expressed as:\\
\scalebox{1}{$P_n =  0.424 + 0.259( \mathit{VNA} + \mathit{TNA} ) + 0.327 ( \mathit{RNF} ) $}\\
\hfill  $+ 0.0008 ( \mathit{VMIR} ) + 0.014 (\mathit{VMIR}) + 0.59 (\mathit{TI})$
\end{comment}

==> tables/fta_basic_original.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Item} & \textbf{Condition} & \textbf{Probability} \\ \hline
a & Instrument Meteorological Conditions & 0.16 \\ \hline
b & Bright Daylight Conditions & 0.7 \\ \hline
c & Encountering General Aviation (GA) Aircraft & 0.79 \\ \hline
d & Intruder is Transponder Equipped & 0.92 \\ \hline
e & Intruder is Mode C Transponder Equipped & 0.61 \\ \hline
f & Risk Ratio for GA Altimetry & 0.317 \\ \hline
g & GA Altimetry Error: Unresolved Component & 0.0143 \\ \hline
h & GA Altimetry Error: Induced Component & 0.0174 \\ \hline
i & Risk Ratio for Maneuvering Intruder & 0.027 \\ \hline
j & Probability of No Track at Time of TA & 0.06 \\ \hline
k & Probability of No Track at Time of RA & 0.03 \\ \hline
l & Risk Ratio for ``Stuck C-Bit" & 0.002 \\ \hline
m & Risk Ratio for Equipment Failure & 0.0001 \\ \hline
n & \begin{tabular}[c]{@{}c@{}}Not Visual Acquisition in Bright Daylight\\ by 15 seconds before CPA\end{tabular} & 0.17 \\ \hline
o & \begin{tabular}[c]{@{}c@{}}Not Visual Acquisition in Bright Daylight\\ by time of RA\end{tabular} & 0.35 \\ \hline
\end{tabular}
\caption{Basic events and their probabilities used in the original TCAS II safety study [citation].}
\label{tab:fta_basic_original}
\end{table}

==> tables/fta_human_vars.tex <==
\begin{table}[ht!]
\centering
\begin{tabularx}{.48\textwidth}{|l|l|X|}
\hline
\textbf{Label} & \textbf{Full Name} & \textbf{Description} \\ \hline
VNA & \begin{tabular}[c]{@{}l@{}}Visual Acquisition; \\ No Avoidance\end{tabular} & \begin{tabular}[c]{@{}l@{}}The pilot makes visual acquisition but \\ does not avoid the NMAC.\end{tabular} \\ \hline
VMIR & \begin{tabular}[c]{@{}l@{}}Visual Acquisition; \\ Maneuvers on \\ Incorrect RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}Although the pilot visually acquires the \\ aircraft, their RA chooses an incorrect \\ maneuver, and the pilot chooses to do \\ the incorrect maneuver.\end{tabular} \\ \hline
RNF & RA; Not Followed & Pilot does not follow their RA. \\ \hline
TNA & TA; No Avoidance & \begin{tabular}[c]{@{}l@{}}Based on the TA alone, the pilot \\ disregardsthe RA and does not \\ avoid NMAC.\end{tabular} \\ \hline
TI & TA; Induces & \begin{tabular}[c]{@{}l@{}}The pilot induces an NMAC by \\ maneuvering on a TA.\end{tabular} \\ \hline
\end{tabularx}
\caption{Plausible human errors as variable factors in the TCAS FTA [citation /ref].}
\label{tab:fta_human_vars}
\end{table}

